Characterizing Python Library Migrations

Developers heavily rely on Application Programming Interfaces (APIs) from libraries to build their software. As software evolves, developers may need to replace the used libraries with alternate libraries, a process known as library migration. Doing this manually can be tedious, time-consuming, and prone to errors. Automated migration techniques can help alleviate some of this burden. However, designing effective automated migration techniques requires understanding the types of code changes required to transform client code that used the old library to the new library. This paper contributes an empirical study that provides a holistic view of Python library migrations, both in terms of the code changes required in a migration and the typical development effort involved. We manually label 3,096 migration-related code changes in 335 Python library migrations from 311 client repositories spanning 141 library pairs from 35 domains. Based on our labeled data, we derive a taxonomy for describing migration-related code changes, PyMigTax. Leveraging PyMigTax and our labeled data, we investigate various characteristics of Python library migrations, such as the types of program elements and properties of API mappings, the combinations of types of migration-related code changes in a migration, and the typical development effort required for a migration. Our findings highlight various potential shortcomings of current library migration tools. For example, we find that 40% of library pairs have API mappings that involve non-function program elements, while most library migration techniques typically assume that function calls from the source library will map into (one or more) function calls from the target library. As an approximation for the development effort involved, we find that, on average, a developer needs to learn about 4 APIs and 2 API mappings to perform a migration, and ... (truncated)

==> lst/lst-migration-yaml.tex <==
\begin{lstlisting}[
    % language=yaml,
    caption=A YAML file describing a migration\sn{do we need this? removing it can save space and then we don't have to explain it; we simply have to say what we add and point the reader to the artifact},
    label=lst:sample-migration-yaml,
    keepspaces=true,
    float=t,
    belowskip=-5mm       
]
repo: rackerlabs/mimic
commit: 5bb494665ce21b645f273bb4597f6dfae861c573
source: characteristic
target: attrs
commit_url: https://github.com/rackerlabs/mimic/commit/5bb49466
files:
- path: mimic/model/customer_objects.py
  code_changes:
  - lines: ["10-12:10"]
    cardinality: many-to-one
    source_program_elements: [decorator, function]
    target_program_elements: [decorator]
    properties: [argument deletion, element name change]
    source_apis: [Attribute, Attribute, attributes]
    target_apis: [s]
- path: mimic/model/flavor_collections.py
  code_changes:
  - lines: ["19-22:19", "90-91:92"]
    cardinality: many-to-one
    source_program_elements: [decorator, function]
    target_program_elements: [decorator]
    properties: [argument deletion, element name change]
    source_apis: [Attribute, attributes]
    target_apis: [s]
  - lines: ["9:9"]
    cardinality: not applicable
    source_program_elements: [import]
    target_program_elements: [import]
    properties: [not applicable]
    source_apis: [characteristic.Attribute, characteristic.attributes]
    target_apis: [attr]
\end{lstlisting}


==> tabs/random-selection-stats.tex <==
% Please add the following required packages to your document preamble:
% \usepackage{booktabs}
\begin{table}[t]
    \centering
    \caption{Distribution of selected SALM migrations in our sample, across domains of the library pairs\sn{should we show unique library pairs in original population and sampled data? to be fair, I don't think we will have space for this table anyways and would probably put it as is (with the extra columns) in the artifact rather than here but we can put it here for now then decide}}
    \label{tab:random-selection-stats}
    \resizebox{0.5\textwidth}{!}{
    \begin{tabular}{@{}lrrr@{}}
        \toprule
        \textbf{Domain}             & \makecell{\textbf{\# Total}\\\textbf{migrations}}  & \makecell{\textbf{\# Selected}\\\textbf{migrations}} & \makecell{\textbf{\%}\\\textbf{Selected}} \\  \midrule
        Utility                     & 364                                                & 85                                                  & 23.35\%              \\
        HTTP Clients                & 342                                                & 80                                                  & 23.39\%              \\
        Crypto                      & 97                                                 & 23                                                  & 23.71\%              \\
        Filesystem                  & 69                                                 & 17                                                  & 24.64\%              \\
        Serialization               & 48                                                 & 12                                                  & 25.00\%              \\
        Web Framework               & 46                                                 & 11                                                  & 23.91\%              \\
        Database                    & 45                                                 & 11                                                  & 24.44\%              \\
        Deep Learning               & 44                                                 & 11                                                  & 25.00\%              \\
        Documentation               & 37                                                 & 9                                                   & 24.32\%              \\
        Auth                        & 30                                                 & 7                                                   & 23.33\%              \\
        Codestyle                   & 30                                                 & 7                                                   & 23.33\%              \\
        Graphic                     & 21                                                 & 5                                                   & 23.81\%              \\
        HTML                        & 16                                                 & 4                                                   & 25.00\%              \\
        Filesystem \& Scientific      & 13                                                 & 4                                                   & 30.77\%              \\
        HTTP Clients \& Crypto        & 13                                                 & 4                                                   & 30.77\%              \\
        Logging                     & 11                                                 & 3                                                   & 27.27\%              \\
        Scientific                  & 10                                                 & 3                                                   & 30.00\%              \\
        Auth \& HTTP Clients          & 8                                                  & 2                                                   & 25.00\%              \\
        Serialization \& Database     & 6                                                  & 2                                                   & 33.33\%              \\
        \makecell[l]{Web Framework \& \\HTTP Clients} & 6                                                  & 2                                                   & 33.33\%              \\
        \makecell[l]{Serialization \& \\Filesystem}   & 4                                                  & 2                                                   & 50.00\%              \\
        \makecell[l]{HTTP Clients \& \\Web Framework} & 3                                                  & 2                                                   & 66.67\%              \\
        Filesystem \& Crypto          & 3                                                  & 2                                                   & 66.67\%              \\
        HTTP Clients \& HTML          & 2                                                  & 2                                                   & 100.00\%             \\
        \makecell[l]{HTTP Clients \& \\Filesystem}    & 1                                                  & 1                                                   & 100.00\%             \\ \toprule
        Total                       & 1269                         & 311                             \\ \bottomrule
    \end{tabular}
    }
\end{table}
